Ehrenfeucht's lemma in set theory

Ehrenfeucht's lemma (1973) asserts that whenever one element of a model of Peano arithmetic is definable from another, then they satisfy different types. We consider here the analogue of Ehrenfeucht's lemma for models of set theory. The original argument applies directly to the ordinal-definable elements of any model of set theory, and in particular, Ehrenfeucht's lemma holds fully for models of set theory satisfying $V=HOD$. We show that the lemma can fail, however, in models of set theory with $V\neq HOD$, and it necessarily fails in the forcing extension to add a generic Cohen real. We go on to formulate a scheme of natural parametric generalizations of Ehrenfeucht's lemma, namely, the principles of the form $EL(A,P,Q)$, which asserts that whenever an object $b$ is definable from some $a\in A$ using parameters in $P$, with $b\neq a$, then the types of $a$ and $b$ over $Q$ are different. We also consider various analogues of Ehrenfeucht's lemma obtained by using algebraicity in place of definability, where a set $b$ is algebraic in $a$ if it is a member of a finite set definable from $a$ (as in Hamkins, Leahy arXiv:1305.5953). Ehrenfeucht's lemma holds for the ordinal-algebraic sets, we prove, if and only if the ordinal-algebraic and ordinal-definable sets coincide. Using similar analysis, we answer two open questions posed by Hamkins and Leahy, by showing that (i) algebraicity and definability need not coincide in models of set theory and (ii) the internal and external notions of being ordinal algebraic need not coincide.

==> EnglishCommands.tex <==
\newcommand{\prooff}[1]{\noindent{\em Proof of {#1}.~}}
\newcommand{\Replacement}{{\sf Replacement}}
\newcommand{\Infinity}{{\sf Infinity}}
\newcommand{\Relativization}{{\sf Relativization}}
\newcommand{\Collection}{{\sf Collection}}
\newcommand{\Powerset}{{\text{\sf Power Set}}}
\newcommand{\Pairing}{{\sf Pairing}}
\newcommand{\UnionAxiom}{{\sf Union}}
\newcommand{\Separation}{{\sf Separation}}
\newcommand{\Foundation}{{\sf Foundation}}
\newcommand{\Identity}{{\sf Identity}}
\newcommand{\SetExistence}{\text{\sf Set Existence}}
\newcommand{\Extensionality}{{\sf Extensionality}} 

==> GeneralCommands.tex <==
\newcommand{\diaschnitt}[2]
        {
          \unitlength#1
          \begin{picture}(1,1)
           \put(0,#2){\line(1,0){1}}
           \put(0,#2){\line(3,5){0.5}}
           \put(1,#2){\line(-3,5){0.5}}
          \end{picture}
         }
\def\diag{\mathop{\vphantom\bigcap\mathchoice
           {\diaschnitt{12pt}{-0.2}\hspace{1pt}}%              display-style
           {\hspace{1pt}\diaschnitt{12pt}{-0.1}\hspace{1.5pt}}%   text-style
           {\diaschnitt{12pt}{-0.2}\hspace{1.5pt}}%             script-style
           {\diaschnitt{12pt}{-0.2}\hspace{1.5pt}}}}%     scriptscript-style
\DeclareMathOperator{\dirlim}{dir\ lim}
\newcommand{\kla}[1]{ {\langle #1 \rangle} }
\newcommand{\anf}[1]{{\text{``}{#1}\text{''}}}
\newcommand{\mathquotes}[1]{{\text{``}}{#1}{\text{''}}}
\newcommand{\goedel}[1]{{\prec}#1{\succ}}%{\,\prec\! #1 \!\succ\,}
\newcommand{\st}{\;|\;}
\newcommand{\mdf}{:=}%{\stackrel{\rm def}{=}}
\newcommand{\dfequiv}{\stackrel{\rm def}{\iff}}
\newcommand{\const}{ {\rm const} }
\newcommand{\dom}{ {\rm dom} }
\newcommand{\ran}{ {\rm ran} }
\newcommand{\otp}{ {\rm otp} }
\newcommand{\Ult}{{\rm Ult}}
\newcommand{\height}{ {\rm ht} }
\newcommand{\length}{ {\rm lh} }
\newcommand{\crit}{ {\rm crit} }
\newcommand{\unt}[1]{\underline{#1}}
\newcommand{\rsupset}{\supsetneqq}
\newcommand{\rsubset}{\subsetneqq}
\newcommand{\sub}{\subseteq}
\newcommand{\super}{\supseteq}
\newcommand{\pO}{ {I\!\!P} }
\newcommand{\bO}{ {I\!\!B} }
\newfont{\ssi}{cmssi12 at 12pt}
\newcommand{\qO}{{\mathbb Q}}
\newcommand{\rO}{ {I\!\!R} }
\newcommand{\oro}{\omega\!\rho}
\newcommand{\dO}{ {I\!\!D} }
\newcommand{\eins}{ {1{\rm\hspace{-0.5ex}l}} }
\newcommand{\gen}{{\rm gen}} % Achtung! Hier kein generischer Filter!!!
\newcommand{\rest}{{\restriction}}
\newcommand{\cf}{ {\rm cf} }
\newcommand{\On}{ {\rm On} }
\newcommand{\Card}{{\rm Card}}
\newcommand{\verl}{{{}^\frown}}%{{\frown\atop }}
\newcommand{\leer}{\emptyset}
\newcommand{\ohne}{\setminus}
\newcommand{\lub}{\mathop{ {\rm lub}} }
\newcommand{\id}{ {\rm id} }
\newcommand{\qedd}[1]{\nopagebreak\hspace*{\fill}$ \Box_{#1} $}
%\newcommand{\qed}{\nopagebreak\hspace*{\fill}$ \Box $\\}
\newenvironment{ea}{\begin{eqnarray}}{\end{eqnarray}}
\newenvironment{ea*}{\begin{eqnarray*}}{\end{eqnarray*}}
\newcommand{\claim}[2]{
     \begin{enumerate}
       \item[{#1}] {\em #2}
     \end{enumerate}}
\newcommand{\js}[3]{ {{\rm J}^{{#1}^{#2}}_{#3}} } % Aufruf:\js{E}{M_i}{\nu_i}
\newcommand{\sig}[1]{{\Sigma_{#1}}}
\newcommand{\Sig}[1]{ {\bf\Sigma}_{#1} }
\newcommand{\sigg}[2]{ \Sigma^{({#1})}_{#2} }
\newcommand{\Sigg}[2]{ {\bf\Sigma}^{({#1})}_{#2} }
\setbox0=\hbox{$\longrightarrow$}
\newcommand{\To}{\longrightarrow}
\newcommand{\emb}[1]{\longrightarrow_{#1} }
\newcommand{\embb}[2]{\longrightarrow^{#1}_{#2}}
\newcommand{\iso}{\stackrel{\sim}{\longleftrightarrow}}
\newcommand{\successors}{\mathrm{succ}}
\newcommand{\lh}{{\rm lh}}
\newcommand{\Lim}{{\rm Lim}}
\newcommand{\pot}{{\cal P}}
\newcommand{\power}{{\cal P}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\gdw}{\,\longleftrightarrow\,}
\newcommand{\ba}{{\bar{a}}}
\newcommand{\bh}{{\bar{h}}}
\newcommand{\bs}{{\bar{s}}}
\newcommand{\bu}{{\bar{u}}}
\newcommand{\bA}{{\bar{A}}}
\newcommand{\bB}{{\bar{B}}}
\newcommand{\bC}{{\bar{C}}}
\newcommand{\bD}{{\bar{D}}}
\newcommand{\bE}{{\bar{E}}}
\newcommand{\bF}{{\bar{F}}}
\newcommand{\bG}{{\bar{G}}}
\newcommand{\bH}{{\bar{H}}}
\newcommand{\bI}{{\bar{I}}}
\newcommand{\bM}{{\bar{M}}}
\newcommand{\bT}{{\bar{T}}}
\newcommand{\bU}{{\bar{U}}}
\newcommand{\bX}{{\bar{X}}}
\newcommand{\bY}{{\bar{Y}}}
\newcommand{\bc}{{\bar{c}}}
\newcommand{\bd}{{\bar{d}}}
\newcommand{\bx}{{\bar{x}}}
\newcommand{\balpha}{{\bar{\alpha}}}
\newcommand{\bbeta}{{\bar{\beta}}}
\newcommand{\bdelta}{{\bar{\delta}}}
\newcommand{\bgamma}{{\bar{\gamma}}}
\newcommand{\bkappa}{{\bar{\kappa}}}
\newcommand{\bnu}{{\bar{\nu}}}
\newcommand{\bmu}{{\bar{\mu}}}
\newcommand{\blambda}{{\bar{\lambda}}}
\newcommand{\btau}{{\bar{\tau}}}
\newcommand{\baeta}{{\bar{\eta}}}
\newcommand{\btheta}{{\bar{\theta}}}
\newcommand{\bpi}{{\bar{\pi}}}
\newcommand{\brho}{{\bar{\rho}}}
\newcommand{\bsigma}{{\bar{\sigma}}}
\newcommand{\bxi}{{\bar{\xi}}}
\newcommand{\bzeta}{{\bar{\zeta}}}
\newcommand{\bGamma}{{\bar{\Gamma}}}
\newcommand{\bard}{{\bar{d}}}
\newcommand{\bare}{{\bar{e}}}
\newcommand{\barf}{{\bar{f}}}
\newcommand{\barg}{{\bar{g}}}
\newcommand{\barm}{{\bar{m}}}
\newcommand{\barn}{{\bar{n}}}
\newcommand{\bt}{{\bar{t}}}
\newcommand{\hs}{{\hat{s}}}
\newcommand{\hE}{{\hat{E}}}
\newcommand{\hT}{{\hat{T}}}
\newcommand{\hkappa}{{\hat{\kappa}}}
\newcommand{\hlambda}{{\hat{\lambda}}}
\newcommand{\tQ}{{\tilde{Q}}}
\newcommand{\tp}{{\tilde{p}}}
\newcommand{\tq}{{\tilde{q}}}
\newcommand{\tih}{{\tilde{h}}}
\newcommand{\ti}{{\tilde{i}}}
\newcommand{\bQ}{{\bar{Q}}}
\newcommand{\bp}{{\bar{p}}}
\newcommand{\bq}{{\bar{q}}}
\newcommand{\bN}{{\bar{N}}}
\newcommand{\tc}{{\tilde{c}}}
\newcommand{\talpha}{{\tilde{\alpha}}}
\newcommand{\tbeta}{{\tilde{\beta}}}
\newcommand{\tdelta}{{\tilde{\delta}}}
\newcommand{\tkappa}{{\tilde{\kappa}}}
\newcommand{\tnu}{{\tilde{\nu}}}
\newcommand{\tlambda}{{\tilde{\lambda}}}
\newcommand{\ttau}{{\tilde{\tau}}}
\newcommand{\teta}{{\tilde{\eta}}}
\newcommand{\tchi}{{\tilde{\chi}}}
\newcommand{\tmu}{{\tilde{\mu}}}
\newcommand{\ttheta}{{\tilde{\theta}}}
\newcommand{\tpi}{{\tilde{\pi}}}
\newcommand{\tpsi}{{\tilde{\psi}}}
\newcommand{\txi}{{\tilde{\xi}}}
\newcommand{\tphi}{{\tilde{\phi}}}
\newcommand{\tsigma}{{\tilde{\sigma}}}
\newcommand{\tA}{{\tilde{A}}}
\newcommand{\tM}{{\tilde{M}}}
\newcommand{\tN}{{\tilde{N}}}
\newcommand{\tD}{{\tilde{D}}}
\newcommand{\tE}{{\tilde{E}}}
\newcommand{\tF}{{\tilde{F}}}
\newcommand{\tT}{{\tilde{T}}}
\newcommand{\tX}{{\tilde{X}}}
\newcommand{\td}{{\tilde{d}}}
\newcommand{\tz}{{\tilde{z}}}
\newcommand{\va}{{\vec{a}}}
\newcommand{\vb}{{\vec{b}}}
\newcommand{\vc}{{\vec{c}}}
\newcommand{\vd}{{\vec{d}}}
\newcommand{\vf}{{\vec{f}}}
\newcommand{\vg}{{\vec{g}}}
\newcommand{\vj}{{\vec{j}}}
\newcommand{\vp}{{\vec{p}}}
\newcommand{\vq}{{\vec{q}}}
\newcommand{\vs}{{\vec{s}}}
\newcommand{\vt}{{\vec{t}}}
\newcommand{\vu}{{\vec{u}}}
\newcommand{\vv}{{\vec{v}}}
\newcommand{\vw}{{\vec{w}}}
\newcommand{\vx}{{\vec{x}}}
\newcommand{\vy}{{\vec{y}}}
\newcommand{\vz}{{\vec{z}}}
\newcommand{\vA}{{\vec{A}}}
\newcommand{\vB}{{\vec{B}}}
\newcommand{\vD}{{\vec{D}}}
\newcommand{\vK}{{\vec{K}}}
\newcommand{\vM}{{\vec{M}}}
\newcommand{\vN}{{\vec{N}}}
\newcommand{\vS}{{\vec{S}}}
\newcommand{\vT}{{\vec{T}}}
\newcommand{\vU}{{\vec{U}}}
\newcommand{\vW}{{\vec{W}}}
\newcommand{\vX}{{\vec{X}}}
\newcommand{\vY}{{\vec{Y}}}
\newcommand{\vr}{{\vec{r}}}
\newcommand{\valpha}{{\vec{\alpha}}}
\newcommand{\vbeta}{{\vec{\beta}}}
\newcommand{\vgamma}{{\vec{\gamma}}}
\newcommand{\vdelta}{{\vec{\delta}}}
\newcommand{\vkappa}{{\vec{\kappa}}}
\newcommand{\vlambda}{{\vec{\lambda}}}
\newcommand{\veta}{{\vec{\eta}}}
\newcommand{\vtau}{{\vec{\tau}}}
\newcommand{\vxi}{{\vec{\xi}}}
\newcommand{\vmu}{{\vec{\mu}}}
\newcommand{\vnu}{{\vec{\nu}}}
\newcommand{\vpi}{{\vec{\pi}}}
\newcommand{\vsigma}{{\vec{\sigma}}}
\newcommand{\vdA}{{\vec{\dot{A}}}}
\newcommand{\vdB}{{\vec{\dot{B}}}}
\newcommand{\seq}[2]{{\langle#1\;|\;}\linebreak[0]{#2\rangle}}
\newcommand{\sequence}[2]{\seq{#1}{#2}}
\newcommand{\mf}[1]{{\mathfrak{#1}}}
\renewcommand{\phi}{\varphi}
\newcommand{\card}[1]{\overline{\overline{#1}}}
\newcommand{\tx}[1]{\;\mbox{\rm #1}\;}
\newcommand{\plusminus}{\pm}
\DeclareMathOperator{\rud}{rud}
\newcommand{\Jonsson}{J\'{o}nsson}
\newcommand{\ZFC}{\ensuremath{\mathsf{ZFC}}}
\newcommand{\ZF}{\ensuremath{\mathsf{ZF}}}
\newcommand{\ZFCm}{\ensuremath{{\ZFC}^-}}
\newcommand{\ZFm}{\ensuremath{{\ZF}^-}}
\newcommand{\KP}{\ensuremath{\mathsf{KP}}}
\newcommand{\AC}{\ensuremath{\mathsf{AC}}}
\newcommand{\DC}{\ensuremath{\mathsf{DC}}}
\newcommand{\AD}{\ensuremath{\mathsf{AD}}}
\newcommand{\MA}{\ensuremath{\mathsf{MA}}}
\newcommand{\MM}{\ensuremath{\mathsf{MM}}}
\newcommand{\MMM}{\ensuremath{\mathsf{MM}^-}}
\newcommand{\PFA}{\ensuremath{\mathsf{PFA}}}
\newcommand{\MAPlusClosed}[1]{\ensuremath{\MA^+({<}#1\text{-closed})}}
\newcommand{\SCH}{\ensuremath{\mathsf{SCH}}}
\newcommand{\V}{\ensuremath{\mathrm{V}}}
\newcommand{\LST}{{\cal L}}
\newcommand{\Funk}[1]{\text{``}\ensuremath{#1}\ \text{is a function''}}
\newcommand{\val}{{\tt val}}
\newcommand{\ers}[2]{({}^{#1}/{}_{#2})}
\newcommand{\bijection}{>\!\!\!\frac{\hphantom{aaaa}}{}\!\!\!\!\!\!>\!\!>}
\newcommand{\onto}{\frac{\hphantom{aaaa}}{}\!\!\!\!\!\!>\!\!>}
\newcommand{\into}{>\!\!\!\frac{\hphantom{aaaa}}{}\!\!\!\!\!\!>}
\newcommand{\forces}{\Vdash}
\newcommand{\proves}{\vdash}
\newcommand{\incomp}{\perp}
\newcommand{\incompatible}{\perp}
\newcommand{\Aut}{\mathop{\hbox{Aut}}}
\newcommand{\TC}{\mathop{\mathsf{TC}}}
\def\<#1>{\langle#1\rangle}
\newcommand{\restrict}{\upharpoonright}
\renewcommand{\P}{{\mathord{\mathbb P}}}
\newcommand{\Q}{{\mathord{\mathbb Q}}}
\newcommand{\R}{{\mathord{\mathbb R}}}
\newcommand{\N}{\mathord{\mathbb{N}}}
\newcommand{\tail}{{\mathord{{\mathbb P}_{\text{\tt tail}}}}}
\newcommand{\dottail}{{\mathord{{\dot{\mathbb P}_{\text{\tt tail}}}}}}
\newcommand{\of}{\subseteq}
\newcommand{\intersect}{\cap}
\newcommand{\union}{\cup}
\newcommand{\Union}{\bigcup}
\newcommand{\cross}{\times}
\newcommand{\compose}{\circ}
\newcommand{\MP}{\ensuremath{\mathsf{MP}}}
\newcommand{\bfMP}{\MP}%{{{\MP}_{_{\boldmath\!\!\!\!\!\!\!\!\sim}}}}
\newcommand{\lt}{{<}}
\newcommand{\closed}[1]{$\lt#1$-closed}
\newcommand{\directed}[1]{$\lt#1$-directed-closed}
\newcommand{\ColNothing}{\mathrm{Col}}
\newcommand{\Col}[1]{\ColNothing(#1)}
\newcommand{\ColStar}[1]{{\ColNothing^*}(#1)}
\newcommand{\dColNothing}{\dot{\ColNothing}}
\newcommand{\dCol}[1]{\dColNothing(#1)}
\newcommand{\MPproper}{\MP_{\mathrm{proper}}}
\newcommand{\MPclosed}[1]{\MP_{<\!#1-\mathrm{closed}}(\{#1\})}
\newcommand{\MPdirected}[1]{\MP_{<\!#1-\mathrm{dir.~cl.}}(\{#1\})}
\newcommand{\MPCol}[1]{\MP_{\Col{#1}}(\{#1\})}
\newcommand{\MPclosedNothing}[1]{\MP_{<\!#1-\mathrm{closed}}}
\newcommand{\MPdirectedNothing}[1]{\MP_{<\!#1-\mathrm{dir.~cl.}}}
\newcommand{\MPColNothing}[1]{\MP_{\Col{\dot{\kappa}}}}
\newcommand{\MPColStar}[1]{\MP_{\ColStar{#1}}(H_{#1}\cup\{#1\})}
\newcommand{\bfMPclosed}[1]{\bfMP_{<\!#1-\mathrm{closed}}(H_{{#1}^+})}
\newcommand{\bfMPdirected}[1]{\bfMP_{<\!#1-\mathrm{dir.~cl.}}(H_{{#1}^+})}
\newcommand{\bfMPCol}[1]{\bfMP_{\Col{#1}}(H_{{#1}^+})}
\newcommand{\bfMPColStar}[1]{\MP_{\ColStar{#1}}(H_{{#1}^+})}
\newcommand{\lfMPclosed}[1]{\bfMP_{<\!#1-\mathrm{closed}}(\leer)}
\newcommand{\lfMPdirected}[1]{\bfMP_{<\!#1-\mathrm{dir.~cl.}}(\leer)}
\newcommand{\lfMPCol}[1]{\bfMP_{\Col{#1}}(\leer)}
\newcommand{\lfMPColStar}[1]{\bfMP_{\ColStar{#1}}(\leer)}
\newcommand{\bfglobalMPclosed}{\bfMP_{\mathrm{closed}}}
\newcommand{\bfglobalMPdirected}{\bfMP_{\mathrm{dir.~cl.}}}
\newcommand{\bfglobalMPCol}{\bfMP_{\Col{}}}
\newcommand{\globalbfMPclosed}{\bfglobalMPclosed}
\newcommand{\globalbfMPdirected}{\bfglobalMPdirected}
\newcommand{\globalbfMPCol}{\bfglobalMPCol}
\newcommand{\Iso}{{\tt Iso}}
\newcommand{\olddiamond}{\diamond}
%\renewcommand{\diamond}{\diamondsuit}
\newcommand{\support}{\mathrm{support}}
\newcommand{\isomorphic}{\cong}
\newcommand{\elementaryIn}{\prec}
\newcommand{\elementary}{\elementaryIn}
\newcommand{\GCH}{\ensuremath{\mathsf{GCH}}}
\newcommand{\CH}{\ensuremath{\mathsf{CH}}}
\newcommand{\CCA}{\ensuremath{\mathsf{CCA}}}
\newcommand{\CF}{{\tt CF}}
\newcommand{\bfSigma}{{\bf \Sigma}}
\newcommand{\OD}{\ensuremath{\mathsf{OD}}}
\newcommand{\HOD}{\ensuremath{\mathsf{HOD}}}
\newcommand{\naturals}{{\mathord{\mathbb{N}}}}
\newcommand{\rationals}{\mathord{\mathbb{Q}}}
\newcommand{\integers}{{\mathord{\mathbb{Z}}}}
\newcommand{\reals}{{\mathord{\mathbb{R}}}}
\newcommand{\keinr}{\hspace*{-\parindent}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\frA}{\mathfrak{A}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Add}{\mathord{\mathrm{Add}}}
\newcommand{\Reg}{\mathsf{Reg}}
\newcommand{\op}{\mathsf{op}}
\newcommand{\lex}{\mathrm{lex}}
\newcommand{\ID}{\mathsf{ID}}
\newcommand{\initsegment}{<_{\mathrm{end}}}
\newcommand{\spcountable}{\mathsf{sp}_{\mathrm{countable}}}
\newcommand{\lift}{\mathop{\uparrow}}
\newcommand{\project}{\mathop{\downarrow}}
\newcommand{\IA}{\mathsf{IA}}
\newcommand{\IATower}[1]{\P^\IA_{<#1}}
\newcommand{\Hull}{\mathcal{H}}
\newcommand{\vdQ}{\vec{\dot{\Q}}}
\newcommand{\contains}{\supseteq}
\newcommand{\isomorphism}{\stackrel{\sim}{\longleftrightarrow}}
\newcommand{\rnk}{\mathop{\mathrm{rnk}}}
\newcommand{\con}{\mathop{\mathsf{con}}}
\newcommand{\possible}{\Diamond}
\newcommand{\necessary}{\Box}
\newcommand{\bairespace}{\mathcal{N}}
\newcommand{\cantorspace}{\mathcal{C}}
\newcommand{\boldSigma}{\utilde{\Sigma}}
\newcommand{\boldPi}{\utilde{\Pi}}
\newcommand{\boldDelta}{\utilde{\Delta}}
\newcommand{\Mantle}{\ensuremath{\mathbb{M}}}
\newcommand{\generic}{\mathsf{g}}
\newcommand{\gMantle}{\ensuremath{\generic\Mantle}}
\newcommand{\gHOD}{\ensuremath{\generic\HOD}}
\newcommand{\IMH}{\ensuremath{\mathsf{IMH}}}
\newcommand{\MirrorPrinciple}{\ensuremath{\reflectbox{$\mathsf{MP}$}}}
\newcommand{\TwoWayMirror}{\ensuremath{\MirrorPrinciple_{\Updownarrow}}}
\newcommand{\UpwardMirror}{\ensuremath{\MirrorPrinciple_{\Uparrow}}}
\newcommand{\BedrockAxiom}{\ensuremath{\mathsf{BA}}}
\newcommand{\GroundAxiom}{\ensuremath{\mathsf{GA}}}
\newcommand{\BA}{\BedrockAxiom}
\newcommand{\GA}{\GroundAxiom}
\newcommand{\NS}{\mathsf{NS}}
\newcommand{\MinP}{\ensuremath{\mathsf{mp}}}
\newcommand{\imh}{\ensuremath{\mathsf{imh}}}
\newcommand{\margin}[1]{\marginpar{\tiny{#1}}}

\newcommand{\Top}{{\rm top}}
\newcommand{\pass}[1]{{#1}^{\rm{passive}}}
\newcommand{\blank}{\textvisiblespace}
\newcommand{\code}[1]{\ulcorner{#1}\urcorner}

\newcommand{\Def}{\mathsf{Def}}

%%%%Difficult names%%%%

\newcommand{\Los}{{\L}{o}{\'s}}
\newcommand{\Loz}{\Los}
\newcommand{\Prikry}{P\v{r}\'{\i}kr\'{y}} 

==> MacroDefinitionsEngl.tex <==
\input{GeneralCommands}
\input{EnglishCommands}
\input{NewTheorems}


==> NewTheorems.tex <==
%
% Theorem Environments
%
\newtheorem{thm}{Theorem}[section]
\newtheorem{cor}[thm]{Corollary}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{obs}[thm]{Observation}
\newtheorem{statement}[thm]{Statement}
\newtheorem{fact}[thm]{Fact}
\newtheorem{conjecture}[thm]{Conjecture}
\theoremstyle{definition}
\newtheorem{defn}[thm]{Definition}
\newtheorem{question}[thm]{Question}
\newtheorem{assumption}[thm]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}[thm]{Remark}
\newtheorem{example}[thm]{Example}

